Melonic limits of the quartic Yukawa model and general features of melonic CFTs

We study a set of large-$N$ tensor field theories with a rich structure of fixed points, encompassing both the melonic and prismatic CFTs observed previously in the conformal limits of other tensor theories and in the generalised Sachdev-Ye-Kitaev (SYK) model. The tensor fields interact via an $O(N)^3$-invariant generalisation of the quartic Yukawa model, $\phi^2\bar{\psi}\psi+\phi^6$. To understand the structure of IR/UV fixed points, we perform a partial four-loop perturbative analysis in $D=3-\epsilon$. We identify the flows between the melonic and prismatic fixed points in the bosonic and fermionic sectors, finding an apparent line of fixed points in both. We reproduce these fixed points non-perturbatively using the Schwinger-Dyson equations, and in addition identify the supersymmetric fixed points in general dimension. Selecting a particular fermionic fixed point, we study its conformal spectrum non-perturbatively, comparing it to the sextic prismatic model. In particular, we establish the dimensional windows in which this theory remains stable. We comment on the structure of large-$N$ melonic CFTs across various dimensions, noting a number of features which we expect to be common to any such theory.

==> 7-OPEdata.tex <==
\section{OPE coefficients and further OPE data} \label{sec:opedata}

A necessary (but not sufficient) condition for a CFT to be unitary is for all OPE coefficients to be real.

We are able to calculate the OPE coefficient for three point functions with two fields and a bilinear with zero and non-zero spin, using the techniques of \cite{Benedetti:2019ikb}.

We need to be able to find the measure, as then we can get the squares of the OPE coefficients from the residues at the poles.



\subsection{Overall procedure}


The four point function in a CFT with a real field of dimension $\Delta_\phi$ can always be written as the following, by doing an OPE of (12) and (34) together:
\[
\begin{aligned}
\left\langle\phi\left(x_1\right) \phi\left(x_2\right) \phi\left(x_3\right) \phi\left(x_4\right)\right\rangle&=\left\langle\phi\left(x_1\right) \phi\left(x_2\right)\right\rangle\left\langle\phi\left(x_3\right) \phi\left(x_4\right)\right\rangle+ & \\
& +\sum_J \int_{\frac{d}{2}-i\infty}^{\frac{d}{2}+i\infty} \frac{d h}{2 \pi i} \frac{1}{1-k(h, J)} \mu_{\Delta_\phi}^d(h, J) G_{h, J}^{\Delta_\phi}\left(x_i\right),
\end{aligned}
\]
with $G_{h, J}^{\Delta_\phi}\left(x_i\right)$ the conformal block, $\mu_{\Delta_\phi}^d(h, J)$ some measure, and $k(h, J)$ the eigenvalues of the two particle irreducible four-point kernel. Note that in the case $d=1$ we have extra contours for $h$ around the even integers.

The OPE expansion is obtained by deforming the integration contour to the right and picking up the poles in the integrand. All the poles coming from the measure and the conformal block are spurious. Specifically, all the poles in the conformal blocks cancel the poles in the coefficient function. Hence:
\[
\left\langle\phi\left(x_1\right) \phi\left(x_2\right) \phi\left(x_3\right) \phi\left(x_4\right)\right\rangle=\left\langle\phi\left(x_1\right) \phi\left(x_2\right)\right\rangle\left\langle\phi\left(x_3\right) \phi\left(x_4\right)\right\rangle+\sum_{m, J} c_{m, J}^2 G_{h_m, J}^{\Delta_\phi}\left(x_i\right),
\]
where $h_{m, J}$ are the poles of $(1-k(h, J))^{-1}$ and the squares of the OPE coefficients are the residues at the poles:
\[
c_{m ; J}^2=-\mu_{\Delta_\phi}^d\left(h_{m, J}, J\right) \operatorname{Res}\left[\frac{1}{1-k(h, J)}\right]_{h=h_{m, J}}=\frac{\mu_{\Delta_\phi}^d\left(h_{m, J}, J\right)}{k^{\prime}\left(h_{m, J}, J\right)},
\]
where the prime denotes a derivative respect to $h$. As we deform the contour to the right, we only pick up the poles with $\operatorname{Re}\left(h_{m, J}\right) \geq d / 2$. If some poles lie on the original integration contour, that is $\operatorname{Re}\left(h_{m, J}\right)=d / 2$, extra care must be taken.

\subsection{Our procedure}

We however will need to generalise this further to include non-scalar, and to arbitrary irreps. Thus, let us first establish what we need to compute. Expanding in the $s$ channel, we can define the connected portion of the 4-point correlator of four operators $\cO_i = \cO_i(x_i)$ (all spin structure is suppressed):
\begin{equation}\begin{aligned}
\expval{\cO_1 \cO_2 \cO_3 \cO_4} = \expval{\cO_1 \cO_2} \expval{\cO_3 \cO_4} + \expval{\cO_1 \cO_2 \cO_3 \cO_4}_{12\to 34}^{full}
\end{aligned}\end{equation}
Now, ignoring subtleties about structures (in the case of scalar fields, where there is only one structure), we in fact have that we have an exact expression in terms of the kernel for the $s$-channel.
\begin{equation}\begin{aligned}
&\expval{\cO_1 \cO_2 \cO_3 \cO_4}_{12\to 34}^{full} = \int d^d x_a d^d x_b \left(\frac{1}{1-K}\right)(x_1, x_2; x_a x_b)\left(G(x_{a3}) G(x_{b4}) + G(x_{b3}) G(x_{a4})\right)\\
&= \int d^d x_a d^d x_b \left(\frac{1}{1-K}\right)(x_1, x_2; x_a x_b)\left[(-1)^{\Sigma_{23}}\<\cO_1(x_a)\cO_3\>\<\cO_2(x_b)\cO_4\>+\<\cO_1(x_a)\cO_4\>\<\cO_2(x_b)\cO_3\>\right]_{MFT}
\end{aligned}\end{equation}

Which, \textbf{up to quibbles about signs}, is clearly equal to
\begin{equation}\begin{aligned}
\expval{\cO_1 \cO_2 \cO_3 \cO_4}_{12\to 34} &= \int d^d x_a d^d x_b \left(\frac{1}{1-K}\right)(x_1, x_2; x_a x_b) \int_{\mathcal{C}} d\cO \rho_{11}^{(s)}(\cO) \Psi_\cO^{(s),11} (x_i)
\end{aligned}\end{equation}
where $\rho_{11}^{(s)}(\cO)$ is the single MFT case.
But we are not dealing with scalar fields. In fact, we have multiple structures.
\begin{equation}\begin{aligned}
\expval{\cO_1 \cO_2 \cO_3 \cO_4}_{12\to 34} &= \int d^d x_a d^d x_b \left(\left(\frac{1}{1-K}\right)(x_1, x_2; x_a x_b)\right) \int_{\mathcal{C}} d\cO \rho_{ab}^{(s)}(\cO) \Psi_\cO^{(s),ab} (x_i)
\end{aligned}\end{equation}
Is the kernel still diagonal when acting on $\Psi_\cO^{(s),ab} (x_i)$? We will have to check this. Further, we need to check that we only need to integrate over $\int_{\mathcal{C}}$, and not also the discrete series that is certainly present in even dimensions.

Our overall tactic will be to perform a MFT decomposition of $\left(G(x_{a3}) G(x_{b4}) + (a \leftrightarrow b)\right)$ into the known conformal blocks. This then will diagonalise the action of the kernel, and then as above we can solve for the conformal blocks.

\subsection{Conformal partial waves and shadow coefficients}

We will mostly follow the presentation of \cite{Albayrak:2020rxh}, except for generalising to arbitrary dimension (and neglecting chirality). We shall assume Euclidean signature. This is covered in a single file in \cite{Albayrak:2021jqx}\url{https://arxiv.org/pdf/2107.13601.pdf}.%

Note that associated to every $\cO$ is a shadow representation $\tilde\cO$ which has dimension $\tilde\delta = d- \delta$, and transforms in the reflected representation $\rho^R$. \textbf{This should be for $\cO=\psi$ be $\tilde{O}^\dagger = \psi^\dagger$}. %

There exists the following conformally invariant pairing%
\begin{align}
&\left(\widetilde{\Psi}^{1234}_{\frac{d}{2}+i\nu,\rho}\ ,\Psi^{1234}_{\frac{d}{2}+i\nu',\rho'}\right)=n_{\frac{d}{2}+i\nu,\rho}\delta_{\rho\rho'}2\pi\delta(\nu-\nu') \qquad (\nu,\nu'\geq0),
\\
&\left(F,G\right)=\int \frac{d^{d}x_{1}...d^{d}x_{n}}{\vol(SO(d+1,1))}F(x_1,...,x_n)G(x_1,...,x_n),
\end{align}
In general we also need to conjugate the operators, but here we introduce the formalism with real operators. Note that because the overall product of operators in any $n$-point function is bosonic, there are no potential sign ambiguities in the $n$-point pairing. (Footnote 9 of \cite{Karateev:2018oml}\url{https://arxiv.org/pdf/1809.05111.pdf}).

The general MFT expansion that we require is the following: in mean field theory we have the factorized correlator
\begin{equation} 
\<\cO_1\cO_2\cO_3\cO_4\>=\<\cO_1\cO_2\>\<\cO_3\cO_4\>
+(-1)^{\Sigma_{23}}\<\cO_1\cO_3\>\<\cO_2\cO_4\>+\<\cO_1\cO_4\>\<\cO_2\cO_3\>.
\end{equation}
The two-point function $\<\cO_i(x_i)\cO_j(x_j)\>$ is only non-zero when $\cO_i=\cO_j^\dagger$, but we will leave this restriction implicit until \cref{eq: generic MFT result}.

We will now expand the MFT four-point function in s-channel partial waves and extract the partial wave expansion coefficient. The first term is automatically separated in the s-channel partial wave expansion ($\Psi^{(s)}$):
\begin{align}
\<\cO_1\cO_2\cO_3\cO_4\>&=\<\cO_1\cO_2\>\<\cO_3\cO_4\>+\int\limits_{\mathcal{C}}d\cO \rho^{(s)}_{ab}(\cO)\Psi^{(s),ab}_{\cO}(x_i), \label{eq:CPW_General}
\\
\Psi^{(s),ab}_{\cO_5}(x_i)&=\int d^{d}x_{5}\<\cO_1\cO_2\cO_5\>^a\<\cO_3\cO_4\widetilde{\cO}_{5}^\dagger\>^{b},
\end{align}

so we can focus on the latter two Wick contractions, which are what we need. However, as described in \cite{Simmons-Duffin:2017nub}, note that we must first subtract off “non-normalizable” contributions coming from the unit operator and scalars with dimensions below $d/2$, which we have ignored here.

\fbox{\parbox{\textwidth}{%
Indeed, we are also having to deal with different three-point function tensor structures, and therefore the inner product between two s-channel partial waves is now a matrix:
\begin{equation}\begin{aligned}\label{eq:etadefinition}
\left(\widetilde{\Psi}^{(s),ab}_{\cO'},\Psi^{(s)cd}_{\cO}\right) =\eta^{(ac)(bd)}_\cO 2\pi\delta(\nu-\nu')\delta_{JJ'},
\end{aligned}\end{equation}
and we can also define the inverse matrix, $\eta_{(ac)(bd)}^\cO \eta ^{(ce)(df)}_\cO=\delta^{e}_{a}\delta^{f}_{b}$.
Note also that in the tilde version we have conjugated all the operators with of course $\tilde{\Psi}_{\Delta,J}^{(s),ab} \equiv \Psi_{\tilde{\Delta},J}^{(s),ab}(\Delta_{i=1234} \to \tilde\Delta_i)$. %
Thus:
\begin{equation}\begin{aligned}
\tilde{\Psi}^{(s),ab}_{{\cO_5}}(x_i)=\int d^{d}x_{5}\<\tilde\cO_1^\dagger \tilde\cO_2^\dagger {\tilde\cO_5}^\dagger\>^a\<\tilde\cO_3^\dagger \tilde\cO_4^\dagger {\cO_5}\>^{b},
\end{aligned}\end{equation}
Note that $\tilde\cO_5^\dagger$ transforms in the conjugate reflected representation, which is equivalent to the same representation in odd dimensions.
}
}
The final contraction, $\<\cO_1\cO_4\>\<\cO_2\cO_3\>$ gives by the orthogonality rule:
\begin{equation}\end{aligned} 
\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<14\>\<23\>} &= \eta^{\cO_5}_{(ac)(bd)}\left(\widetilde{\Psi}^{(s),cd}_{\cO_5},\<\cO_1\cO_4\>\<\cO_2\cO_3\>\right)
\\ &= \eta^{\cO_5}_{(ac)(bd)}\int d^{d}x_{1}\cdots d^{d}x_{5}\<\widetilde{\cO}_{1}\widetilde{\cO}_{2}\widetilde{\cO}_{5}\>^c\<\widetilde{\cO}_3\widetilde{\cO}_4\cO_5\>^d\<\cO_1\cO_4\>\<\cO_2\cO_3\>
\\ &= \eta^{\cO_5}_{(ac)(bd)} (-1)^{\Sigma_{11}+\Sigma_{22}}S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{f}([\widetilde{\cO}_2]\cO_{1}\cO_5)\left(\<\widetilde{\cO}_{1}\widetilde{\cO}_{2}\widetilde{\cO}_{5}\>^c,\<\cO_2\cO_1\cO_5\>^f\right),
\end{aligned}\end{equation} 

The first contraction $(-1)^{\Sigma_{23}}\<\cO_1\cO_3\>\<\cO_2\cO_4\>$ gives a similar result:
\begin{equation}\begin{aligned}
\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<13\>\<24\>}&=(-1)^{\Sigma_{23}} \eta^{\cO_5}_{(ac)(bd)}\left(\widetilde{\Psi}^{(s),cd}_{\cO_5},\<\cO_1\cO_3\>\<\cO_2\cO_4\>\right)
\\
&=(-1)^{\Sigma_{23}+\Sigma_{11}+\Sigma_{22}}\eta^{\cO_5}_{(ac)(bd)}S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{f}(\cO_1[\widetilde{\cO}_{2}]\cO_5)\left(\<\widetilde{\cO}_{1}\widetilde{\cO}_{2}\widetilde{\cO}_{5}\>^{c},\<\cO_1\cO_2\cO_5\>^f\right).
\end{aligned}\end{equation}

The full result in MFT is then in full generality
\begin{equation}\begin{aligned}
\rho^{(s),\text{MFT}}_{ab}(\cO)=\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\rho_{ab}^{(s)}(\cO)\bigg|_{\<14\>\<23\>}+\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}\rho_{ab}^{(s)}(\cO)\bigg|_{\<13\>\<24\>}, \label{eq: generic MFT result}
\end{aligned}\end{equation}
where $\hat{\delta}_{\cO_1\cO_2}$ is $1$ if the operators are the same ($\Delta_1=\Delta_2$, and $\rho_1 = \rho_2$), and is otherwise $0$.%
We need to be able to calculate this!

We already have the shadow transforms, so it remains to calculate the $\eta$s and the inner products. 

How do these quantities map on to the quantities described earlier? Well clearly for the case of one structure $\rho^{(s)}_{11}(\mathcal{O}) = \rho^0 (\Delta, J)$.



Now let us define the conformal three-point pairing $t_0$%
\begin{equation}\begin{aligned}
(t_{0,125})^{cf}=t_0^{cf}(\cO_1,\cO_2,\cO_5) = \left(\<\widetilde{\cO}_{1}\widetilde{\cO}_{2}\widetilde{\cO}_{5}\>^{c},\<\cO_1\cO_2\cO_5\>^f\right)
\end{aligned}\end{equation}
comparing with \cite{Liu:2018jhs} which yields

\begin{equation}\begin{aligned}
\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<14\>\<23\>} &= \eta^{\cO_5}_{(ac)(bd)} (-1)^{\Sigma_{11}+\Sigma_{22}}S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{f}([\widetilde{\cO}_2]\cO_{1}\cO_5)(t_{0,(125)})^{cf},\\
\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<13\>\<24\>}&=(-1)^{\Sigma_{23}+\Sigma_{11}+\Sigma_{22}}\eta^{\cO_5}_{(ac)(bd)}S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{f}(\cO_1[\widetilde{\cO}_{2}]\cO_5) (t_{0,(125)})^{cf}\\
\rho^{(s),\text{MFT}}_{ab}(\cO_5)&=\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<14\>\<23\>}+\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}\rho_{ab}^{(s)}(\cO_5)\bigg|_{\<13\>\<24\>},\\
&=\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\left(\eta^{\cO_5}_{(ac)(bd)} (-1)^{\Sigma_{11}+\Sigma_{22}}S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{f}([\widetilde{\cO}_2]\cO_{1}\cO_5)(t_{0,(125)})^{cf}\right)\\
    &\quad +\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}\left((-1)^{\Sigma_{23}+\Sigma_{11}+\Sigma_{22}}\eta^{\cO_5}_{(ac)(bd)}S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{f}(\cO_1[\widetilde{\cO}_{2}]\cO_5) (t_{0,(125)})^{cf}\right),\\
&=\eta^{\cO_5}_{(ac)(bd)} (t_{0,(125)})^{cf} (-1)^{\Sigma_{11}+\Sigma_{22}} %
     \left\{\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\left(S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{f}([\widetilde{\cO}_2]\cO_{1}\cO_5)\right)\right.\\
      &\left.\quad +\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}(-1)^{\Sigma_{23}}\left( S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{f}(\cO_1[\widetilde{\cO}_{2}]\cO_5) \right)\right\}, \label{eq:rhosMFTDef}
\end{aligned}\end{equation}

Then, finally, we have that the OPE coefficients are:
\begin{equation}\begin{aligned}
P_{ab}^{s}(\cO_5) &= \lambda_{125,a}\lambda_{345,b} = (-1)^{\Sigma_{55}+1} \mathrm{Res}_{\Delta=\Delta_5} \rho_{ac}^{(s),MFT}(\cO_5) S^c_b(\cO_3 \cO_4 [\tilde\cO_5]|_{J=J_5}\\
& \equiv -\mathrm{Res}_{\Delta} \, C_{ab\<\cO_1 \cO_2 \cO_5\>\<\cO_3 \cO_4 \cO_5\>}^{\text{MFT}}|_{J=J_5} %
\end{aligned}\end{equation}

It now remains to calculate the three components: $S$ (in an appendix), $\eta$, and $t_0$.


\subsection{\texorpdfstring{$\eta$}{eta} calculation}

These seem to be done in full generality by \cite{Albayrak:2020rxh}.

\begin{equation}\begin{aligned}
\text{Want} & \left(\widetilde{\Psi}^{(s),ab}_{\cO_5},\Psi^{(s)cd}_{\cO_6}\right) =\eta^{(ac)(bd)}_\cO 2\pi\delta(\nu-\nu')\delta_{JJ'},\\
\tilde\Psi^{(s),ab}_{\cO_5}(x_i)&=\int d^{d}x_{5}\<\tilde\cO_1^\dagger\tilde\cO_2^\dagger\tilde\cO_5^\dagger\>^a\<\tilde\cO_3^\dagger\tilde\cO_4^\dagger\cO_5\>^{b},\\
\Psi^{(s),cd}_{\cO_6}(x_i)&=\int d^{d}x_{6}\<\cO_1\cO_2\cO_6\>^c\<\cO_3\cO_4\widetilde{\cO}_{6}^\dagger\>^{d},
\end{aligned}\end{equation}
where we have paired up the Lorentz indices (including spinor indices) of $\cO_5,\cO_6$ with their conjugates, as $(\tilde{\cO}_5^\dagger)^{\alpha \cdots}(\cO_5)_{\alpha\cdots}$. Hence we are calculating:
\begin{equation}\begin{aligned}
&\int \frac{d^d x_1 \ldots d^d x_4}{\vol(\SO(d+1,1))} \tilde\Psi^{(s),ab}_{\cO_5}(x_i)\Psi^{(s),cd}_{\cO_6}(x_i)\\
=& \int \frac{d^d x_1 \ldots d^d x_6}{\vol(\SO(d+1,1))} \<\tilde\cO_1^\dagger\tilde\cO_2^\dagger\tilde\cO_5^\dagger\>^a\<\tilde\cO_3^\dagger\tilde\cO_4^\dagger\cO_5\>^{b} \<\cO_1\cO_2\cO_6\>^c\<\cO_3\cO_4\widetilde{\cO}_{6}^\dagger\>^{d}
\end{aligned}\end{equation}
where all indices are paired canonically. We know that the result here should be proportional to $\delta(s_6-s_5)$, where $\Delta_{5,6} = \frac{d}{2} + i s_{5,6}$, with $s_5, s_6\ge 0$.

\cite{Albayrak:2020rxh} gives very immediately that:
\begin{equation}\begin{aligned}\label{eq:Phipairing}
\left(\Psi^{\tilde{(s)},ab}_{\cO_5},\Psi^{(s)cd}_{\cO_6}\right) = \frac{\delta_{O_5 \tilde\cO_6} (-1)^{2l_6}}{\mu(\cO_6)} \left(\< \tilde\cO_1 \tilde\cO_2 \tilde\cO_6\>^a \cdot \<\cO_1 \cO_2 \cO_6\>^c\right) \left(\< \tilde\cO_3 \tilde\cO_4 \cO_6\>^b \cdot \<\cO_3 \cO_4 \tilde\cO_6\>^d\right)
\end{aligned}\end{equation}
where $\tilde{(s)}$ indicates that $\cO_{i=1,\ldots,4}$ are replaced by $\tilde{\cO}_i$, and $\delta_{\cO \cO'} = \delta_{\Delta \Delta'} \delta_{ss'}$, where $\delta_{\Delta \Delta'}$ = PROBABLY $2\pi \delta(s-s')$.

We want a slightly more general case, with daggers, which is given by 2.39 (and derived in the appendix A) of \cite{Karateev:2018oml}:
\begin{equation}\begin{aligned}
\left(\Psi^{(s),\cO_i,ab}_{\cO},\Psi^{(s),\cO_i^\dagger,cd}_{\tilde\cO^{\prime\dagger}}\right) = \frac{\delta_{\cO\cO'}}{\mu(\cO)} \left(\<\cO_1 \cO_2 \cO\>^a \cdot \<\tilde\cO_1^\dagger \tilde\cO_2^\dagger \tilde\cO^\dagger\>^c\right) \left(\< \cO_3 \cO_4 \tilde\cO^\dagger\>^b \cdot \<\tilde\cO_3^\dagger \tilde\cO_4^\dagger \cO\>^d\right)
\end{aligned}\end{equation}

\subsection{Plancherel measure}

We also need to define the Plancherel measure, (see C.1 of 2006):
\begin{equation}\begin{aligned}
\mu\left(\Delta, \rho_{\mathrm{irrep}}\right)
\end{aligned}\end{equation}
We can get the base case $\rho=$scalar from the pairing of scalar 2-point functions
\begin{equation}\begin{aligned}
\left(\<\phi_1 \phi_2\>\<\tilde\phi_1 \tilde\phi_2\>\right) = \int \frac{d^d x_1 d^d x_2}{\vol(\SO(d+1,1))}\<\phi_1 \phi_2\>\<\tilde\phi_1 \tilde\phi_2\> = \int \frac{d^d x_1 d^d x_2}{\vol(\SO(d+1,1))} \frac{1}{(x_{12}^2)^{d}}
\end{aligned}\end{equation}
FP gauge fixing to $0$,$\infty$ (hence the $2^d$, and the stabiliser group left over), we obtain
\begin{equation}\begin{aligned}
\left(\<\phi_1 \phi_2\>\<\tilde\phi_1 \tilde\phi_2\>\right) = \frac{1}{2^d\vol(\SO(1,1))\vol(\SO(d))}
\end{aligned}\end{equation}
Now, we use their convention that $SO(n)$ has volume $=\vol(\SO(n-1))\vol(S^{n-1})$, and $\vol(SO(2)) = 2\pi$. This agrees with their version, since they evaluate $2^d \vol(\SO(d))|_{d=3} = 2^d \vol(\SO(2)) \vol(S^2) = 2^3\cdot 2\pi \cdot 4\pi = 64 \pi^2$.

What about higher spins? \cite{Karateev:2018oml} appears to have the more general answers for solving the pairing. 

However, essentially we have that the measure is:
\begin{equation}\begin{aligned}
\mu(\cO) = \frac{\vol(\SO(1,1))}{\mathcal{N}_O} 
\left(\<\cO \cO\>\cdot \<\tilde\cO \tilde\cO\>\right)
\end{aligned}\end{equation}
where we have the usual $\mathbf{S}^2[\cO]= \mathcal{N}_\cO \cO$. For an arbitrary $SO(d)$ irrep with weight $\mathbf{m}_{d}$, we first define the associated (formal) $SO(d+1,1)$ weight $\mathbf{m}_{d+2}=(-\Delta, \mathbf{m}_d)$, which is a vector of length $n+1\equiv \lfloor d/2 \rfloor$+1. Then:
\begin{equation}\begin{aligned}
\mu(\Delta, \mathbf{m}_d) = (-1)^n 2\pi \frac{\dim(\mathbf{m}_{d+2})}{\vol(\SO(d+2))} \times \begin{cases} 1 & d=2n,\\ -\cot (\pi(\Delta-(\mathbf{m}_d)_1)) & d=2n+1\end{cases}
\end{aligned}\end{equation}
where the $\dim(\mathbf{m}_{d+2})$ should be understood as a formal rational function given by the standard formula for the dimension of an $\SO(d+2)$ irrep.

Sadly we have lost the nice interpretation of continuous dimension.

\subsection{Evaluation of \texorpdfstring{$\eta$}{eta}}

Comparing \eqref{eq:Phipairing} with our definition of $\eta$, \eqref{eq:etadefinition}, it is manifest that the lowered $\eta$ must be:
\begin{equation}\begin{aligned}
\eta_{(ac)(bd)}^{\cO_5} = (-1)^{2l_5}\mu(\cO_5) \left(\left(\< \tilde\cO_1 \tilde\cO_2 \tilde\cO_5\>^a \cdot \<\cO_1 \cO_2 \cO_5\>^c\right) \left(\< \tilde\cO_3 \tilde\cO_4 \cO_5\>^b \cdot \<\cO_3 \cO_4 \tilde\cO_5\>^d\right)\right)^{-1}
\end{aligned}\end{equation}
where the matrices are inverted. 
Recall that 
\begin{equation}\begin{aligned}
(t_{0,125})^{cf}=t_0^{cf}(\cO_1,\cO_2,\cO_5) = \left(\<\widetilde{\cO}_{1}\widetilde{\cO}_{2}\widetilde{\cO}_{5}\>^{c},\<\cO_1\cO_2\cO_5\>^f\right)
\end{aligned}\end{equation}
We therefore observe
\begin{equation}\begin{aligned}
\eta_{(ac)(bd)}^{\cO_5} = (-1)^{2l_5}\mu(\cO_5) \left((t_{0,125}^{ac}) (t_{0,34\tilde{5}}^{bd})\right)^{-1}, \quad (t^{ab})^{-1}t^{cd} = \delta_a^c \delta_b^d
\end{aligned}\end{equation}
Let us therefore instead write $(t_{i}^{ac})^{-1}$ as $(t^{-1}_{i})_{ac}$ Which, plugging back into \eqref{eq:rhosMFTDef} we calculate to be
\begin{equation}\begin{aligned}
\rho^{(s),\text{MFT}}_{ab}(\cO) & =(-1)^{2l_5}\mu(\cO_5) \left((t_{0,125}^{ac}) (t_{0,34\tilde{5}}^{bd})\right)^{-1} (t_{0,(125)})^{cf} (-1)^{\Sigma_{11}+\Sigma_{22}}\\       
 &\quad \left\{\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\left(S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{f}([\widetilde{\cO}_2]\cO_{1}\cO_5)\right)\right.\\
  &\left.\quad +\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}(-1)^{\Sigma_{23}}\left( S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{f}(\cO_1[\widetilde{\cO}_{2}]\cO_5) \right)\right\},
\end{aligned}\end{equation}
We can then cancel the $t_{0,125}$s to obtain a $\delta_a^f$:
\begin{equation}\begin{aligned}
\rho^{(s),\text{MFT}}_{ab}(\cO) & =(-1)^{2l_5}\mu(\cO_5) \left(t_{0,34\tilde{5}}^{bd}\right)^{-1} (-1)^{\Sigma_{11}+\Sigma_{22}}\\       
 &\quad \left\{\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\left(S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{a}([\widetilde{\cO}_2]\cO_{1}\cO_5)\right)\right.\\
  &\left.\quad +\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}(-1)^{\Sigma_{23}}\left( S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{a}(\cO_1[\widetilde{\cO}_{2}]\cO_5) \right)\right\},
\end{aligned}\end{equation}
Since we defined $C = \rho S$, we have that
\begin{align}
& C_{ab\<\cO_1 \cO_2 \cO_5\>\<\cO_3 \cO_4 \cO_5\>}^{\text{MFT}} =\rho^{(s),\text{MFT}}_{ac}(\cO)   S^c_b(\cO_3 \cO_4 [\tilde\cO_5])\\
&=(-1)^{2l_5}\mu(\cO_5) \left(t^{-1}_{0,34\tilde{5}}\right)_{cd} (-1)^{\Sigma_{11}+\Sigma_{22}}\\       
 &\quad \left\{\hat{\delta}_{\cO_1\cO_4}\hat{\delta}_{\cO_2\cO_3}\left(S^{d}_{e}(\widetilde{\cO}_2[\widetilde{\cO}_1]\cO_5)S^{e}_{a}([\widetilde{\cO}_2]\cO_{1}\cO_5)\right)\right.\\
  &\left.\quad +\hat{\delta}_{\cO_2\cO_4}\hat{\delta}_{\cO_1\cO_3}(-1)^{\Sigma_{23}}\left( S^{d}_{e}([\widetilde{\cO}_{1}]\widetilde{\cO}_{2}\cO_5)S^{e}_{a}(\cO_1[\widetilde{\cO}_{2}]\cO_5) \right)\right\}S^c_b(\cO_3 \cO_4 [\tilde\cO_5]). \label{eq:CfullMFTDef}
\end{align}

















==> 99-1-OPEdataConventions.tex <==
\section{Our model conventions}

We will be using embedding space $X$, with polarizations $S$; a review in 3D is given in \url{https://arxiv.org/pdf/2006.07374.pdf} \cite{Albayrak:2020rxh}; a more general review can be found in \url{https://arxiv.org/pdf/1706.02835.pdf} \cite{Isono:2017grm}. Likewise, $(x,s)$ for physical space. We will work in Euclidean space. All indices will be spinor indices.
Our conventions will be that for some operator $\mathcal{O}$, we have:
\begin{align}
    \mathcal{O}_{\Delta,l}(x,s) = s_{\alpha_1}\ldots s_{\alpha_{2l}} \mathcal{O}^{\alpha_1 \ldots \alpha_{2l}},\,
    \mathcal{O}_{\Delta,l}(X,S) = S_{I_1}\ldots S_{I_{2l}} \mathcal{O}^{I_1 \ldots I_{2l}},
\end{align}
We will normalise the two-point functions as:
\begin{equation}
    \expval{\psi(P_1, \bar{S}_1) \bar{\psi}(P_2,S_2)} = \frac{\braket{1|2}}{(P_{12})^{\Delta +1/2}} \quad \implies \quad \expval{\psi(x) \bar{\psi}(x')} = \frac{\mel{1}{x-x'}{2}}{\abs{x-x'}^{2\Delta +1}}
\end{equation}
Three-point functions of two spinors and one symmetric tensor (\url{https://arxiv.org/pdf/1706.02835.pdf}):
\begin{align}
\lan \Psi_1(P_1,S_1) \bar\Psi_2(P_2,S_2) O^{(\ell)}(P_3,Z_3) \ran,
\end{align}
where $\Psi_{i}$ has dimension $\De_{i}$ and $O$ has dimension $\De_3$ and integer spin $\ell$. We parametrise the correlation function as
\begin{align}
C_{\frac{1}{2}\frac{1}{2}\ell}(\De_1,\De_2,\De_3)
&:=
\lan \Psi_1(P_1,S_1) \bar\Psi_2(P_2,\bar S_2) O^{(\ell)}(P_3,Z_3) \ran
\nn\\
&=
f_{\frac{1}{2}\frac{1}{2}\ell}(P_i,\bar S_1,S_2,Z_3)
P_{12}^{-\frac{\Sig_{12}-\De_3+1-\ell}{2}}
P_{23}^{-\frac{\De_3-\De_{12}+\ell}{2}}
P_{31}^{-\frac{\De_3+\De_{12}+\ell}{2}}.
\label{1/21/2l}
\end{align}
with $\Sigma_{ij} = \Delta_i + \Delta_j$, and $\Delta_{ij} = \Delta_i - \Delta_j$.
The homogeneity conditions from embedding space are: $\Psi(aP, bS) = a^{-\Delta-half} b \Psi(P,S)$, $T_{M_{1}\ldots M_\ell}(\lambda P) = \lambda^{-\Delta} T_{M_1 \ldots M_\ell}(P)$. 
The transversality condition on $O^\ell$, fully contracted with a polarization vector $Z$ is: $T(P,Z) = T(P, Z+\alpha P) \forall \alpha$. These constrain as follows: $f_{\frac{1}{2}\frac{1}{2}\ell}$
\begin{align}
&{} 
f_{\frac{1}{2}\frac{1}{2}\ell}(\lm_iP_i, a\bar S_1, bS_2, cZ_3) 
= \lm_3^\ell abc^\ell \, f_{\frac{1}{2}\frac{1}{2}\ell}(P_i, \bar S_1, S_2, Z_3), 
\label{homo1/21/2l} \\
&{}
f_{\frac{1}{2}\frac{1}{2}\ell}(P_i, \bar S_1, S_2, Z_3) 
= f_{\frac{1}{2}\frac{1}{2}\ell}(P_i, \bar S_1, S_2, Z_3+\al P_3)
\quad \mbox{ for any } \, \al.
\label{transv1/21/2l}
\end{align}
Note that the homogeneity condition implies that $f_{\frac{1}{2}\frac{1}{2}\ell}$ 
must have only one spinor quadratics with $\bar S_1, S_2$.
Solving, we find in odd dimension that the results are combinations of the following three-point structures,\begin{align}
f^{(1)}_{\frac{1}{2}\frac{1}{2}\ell} 
&:= 
\lan \bar S_1S_2\ran I_3^\ell, \\
f^{(2)}_{\frac{1}{2}\frac{1}{2}\ell}
&:= 
\lan \bar S_1P_3S_2\ran I_3^\ell \sqrt{\frac{P_{12}}{P_{13}P_{23}}}, \\
\text{Not }\cancel{f^{(3)}_{\frac{1}{2}\frac{1}{2}\ell} }
&:= 
I_3^{\ell-1} J_3^{(1)}, \text{ due to linear dependence: } 2f^{(2)} = f^{(4)}-f^{(3)} \\
f^{(4)}_{\frac{1}{2}\frac{1}{2}\ell}
&:= 
I_3^{\ell-1} J_3^{(2)}, \\
f^{(5)}_{\frac{1}{2}\frac{1}{2}\ell} 
&:= I_3^{\ell-1} \lan \bar S_1Z_3P_3S_2\ran,
\end{align}
where we introduced several scalar quantities, 
all of which are defined to be invariant under the replacement $Z_3 \to Z_3+\al P_3$,
\begin{align}
I_3 &:= \frac{P_{23}(P_1.Z_3)-P_{13}(P_2.Z_3)}{P_{12}}, \\
J_3^{(1)} &:= \left[ \lan \bar S_1Z_3S_2\ran P_{13} + 2\lan \bar S_1P_3S_2\ran P_1.Z_3 \right]
\sqrt{\frac{P_{23}}{P_{12}P_{13}}}, \\
J_3^{(2)} &:= \left[ \lan \bar S_1Z_3S_2\ran P_{23} + 2\lan \bar S_1P_3S_2\ran P_2.Z_3 \right]
\sqrt{\frac{P_{13}}{P_{12}P_{23}}}.
\end{align}
For even-dimensional conformal field theories, 
the conditions \eqref{homo1/21/2l} and \eqref{transv1/21/2l} yield five more solutions,
which we denote by $f^{(i+5)}_{\frac{1}{2}\frac{1}{2}\ell}$ $(1 \leq i \leq 5)$, 
defined by replacing $\bar S_1$ in $f^{(i)}_{\frac{1}{2}\frac{1}{2}\ell}$ by $\bar S_1\Ga$, with $\Ga$ the chirality matrix for (d + 2)-dimensional Dirac matrices.

Let us now shadow transform $S[\psi]\psi O^\ell$ for the conformal structure $f^{(1)}_{\frac{1}{2}\frac{1}{2}\ell}$. To do this, we will need the two-point correlator. We will need to calculate $t_0$ for our case, for which we will follow \cite{Albayrak:2020rxh}, below.



To do these computations, we use embedding space: 

\subsection{Rules of embedding space}

As a reminder, here are the rules of embedding space. The dot product is:
\begin{equation}\begin{aligned}
A^M =(A^\mu, A^+, A^-), \quad A \cdot B = A^\mu B_\mu -\half (A^+ B^- + A^- B^+)
\end{aligned}\end{equation}
If the thing being contracted is a symmetric traceless $J$-tensor, and we want to calculate:
\begin{equation}\begin{aligned}
\<\cdots \phi_{\mu\cdots \nu}\> \<\phi^{\mu\cdots \nu}\dots \>
\end{aligned}\end{equation}
Let us first consider instead $\Phi(x)= Z^M \cdots Z^N \Phi_{M\cdots N}$. We can recover the original tensor field in the physical space by replacing coordinates $X^M=(X^\mu,X^+,X^-)$ by $P^M(x)$, and multiplying each (lowered) vector index of the embedding space tensor field by $\partial P^M(x)/\partial x^\mu$. %
In particular, this latter quantity is:
\begin{equation}\begin{aligned}
P^M(x) = (x^\mu, 1, x^2)\text{ and so } \pd{P^M(x)}{x^\mu} = \begin{pmatrix} \delta^M_\mu & \mathbf{0} & 2x_\mu\end{pmatrix}
\end{aligned}\end{equation}
This can be seen to come from $Z^\mu_{z,x} = (z^\mu, 0, 2 x \cdot z)$, which of course satisfies $Z_{z,x} \cdot P(x) =0$ as required. Thus, we have the relation:
\begin{equation}\begin{aligned}
\Phi_{M \cdots N}(P) &= \mathcal{D}_M \cdots \mathcal{D}_N \Phi(P,Z)\\
\phi_{\mu\cdots \nu}(x) &= \pd{P^M(x)}{x^\mu} \cdots \pd{P^N(x)}{x^\nu}\Phi_{M \cdots N}(P(x))
\end{aligned}\end{equation}
Note that this agrees with the standard scalar case $\phi(x) = (X^+)^\Delta \Phi(X(x))$, because if we simply replace $X$ by $X(x)$, then $X^+ =1$.


The structures that we can easily find in the embedding space are $F$ and $G$ in the following:
\begin{equation}\begin{aligned}
\< \cdots \Phi\> = Z_M \cdots Z_N F^{M\cdots N}(P), \quad \<\Phi \cdots \> = W_M \cdots W_N G^{M\cdots N}(P) \< \Phi \cdots\>
\end{aligned}\end{equation}
these $F$ and $G$ are by definition symmetric, but not necessarily traceless. (However, the F and G that would be constructed by \cite{Isono:2017grm} (A.6), or \cite{Costa:2011mg} (3.7) would indeed be traceless).
How then can we evaluate
\begin{equation}\begin{aligned}
\<\cdots \phi_{\mu\cdots \nu}\> \<\phi^{\mu\cdots \nu}\dots \>
\end{aligned}\end{equation}
The obvious starting point would be $g_{M_1 N_1} \cdots g_{M_J N_J} F^{M_1\cdots M_J}G^{N_1\cdots N_J}$, i.e. contracting with two structures with the $(D+2)$-dimensional metric. However, that is not quite right, as from the above, we know that 
\begin{equation}\begin{aligned}
\<\cdots \phi_{\mu\cdots \nu}\> = \left(\pd{P^M(x)}{x^\mu} \cdots \pd{P^N(x)}{x^\nu} F_{M\cdots N}(P(x)) - \text{traces}\right)
\end{aligned}\end{equation}
and likewise for $\<\phi^{\mu\cdots \nu}\dots \>$. But since all the traces take the form of $\propto g^{AB} g^{CD}F^M{}_M{}^N{}_{NOP\cdots}$, they will vanish on being contracted with the traceless other bracket. Hence, all of the terms vanish on one side:
\begin{equation}\begin{aligned}
&\<\cdots \phi_{\mu\cdots \nu}(x)\> \<\phi^{\mu\cdots \nu}(y)\dots \> = g^{\mu_1 \nu_1} \cdots g^{\mu_J\nu_J} \left(\pd{P^{M_1}(x)}{x^{\mu_1}} \cdots \pd{P^{M_J}(x)}{x^{\mu_J}} F_{M_1\cdots M_J}(P(x))\right)\\
&\times \left(\pd{P^{N_1}(y)}{y^{\nu_1}} \cdots \pd{P^{N_J}(y)}{y^{\nu_J}} G_{N_1\cdots N_J}(P(y)) - \text{traces}\right) 
\end{aligned}\end{equation}
We need only really consider
\begin{equation}\begin{aligned}
A^{MN}= g^{\mu\nu} \pd{P^{M}(x)}{x^{\mu}} \pd{P^{N}(y)}{y^{\nu}} =\begin{pmatrix} g^{mn} & \mathbf{0} & 2 y^m\\ \mathbf{0} & 0 & 0\\ 2x^n & 0 & 4 x\cdot y\end{pmatrix}\text{, with }m=M, n=N.
\end{aligned}\end{equation}
What exactly is this equal to? See the file \verb{OPEco}, page 25. However, we will likely want to use some form of transversality to make the terms vanish (see \url{https://arxiv.org/pdf/1107.3554.pdf}, 3.32).

\subsection{Simple replacement rules}
Simple replacement rules from \cite{Costa:2011mg}, (3.37):
\begin{equation}\begin{aligned}
Z_1 \cdot Z_2 \to z_1 \cdot z_2, \quad P_{12}=-2 P_1 \cdot P_2 = x_{12}^2\\
P_1 \cdot Z_2 \to z_2 \cdot x_{12}, \quad P_i \cdot Z_j \to z_j \cdot x_{ij} = - z_j \cdot x_{ji}\text{ (no sum)}
\end{aligned}\end{equation}

And further%

\begin{equation}\begin{aligned}
&\bar{S}_i = (\bar{s}_i, -\bar{s}_i x_i^\rho \gamma_\rho \delta^{-1}), S_i = \begin{pmatrix}x_i^\rho \gamma_\rho s_i\\ \delta s_i\end{pmatrix}\\
&\psi(x_i, s_i) = \bar{s}_i \psi(x_i), \quad \<\bar{S}_1 S_2\> \to \bar{s}_1(\not{x}_2 - \not{x}_1)s_2\\
&\<\bar{S}_1 \not{P}_y S_2\> \to \bar{s}_1(\not{y}-\not{x}_1)(\not{x}_2 -\not{y})s_2\\
&\<\bar{S}_1 \not{P}_y \not{P}_z S_2\> \to \bar{s}_1 (\not{y}-\not{x_1})(\not{y}-\not{z})(\not{z}-\not{x}_2)s_2\\
&\text{For }\Xi_x^M=(\xi^\mu, 0, 2 x \cdot \xi),\\
&\leadsto\bar{S}_a\not\Xi_x S_b = \bar{S}_a\Xi_x^M \Gamma_M S_b = \bar{s}_a\left[\not{\xi}(\not{b}-\not{x}) + (\not{a}-\not{x})\not{\xi}\right]s_b\\
&\leadsto\bar{S}_a\not\Xi_x \not{P}_y S_b = \bar{s}_a\left[\not{\xi}(\not{b}-\not{x}) + (\not{a}-\not{x})\not{\xi}\right]s_b\\
&\<\bar{S}_1 \not{P}_y \not{P}_z S_2\> \to \bar{s}_1 (\not{y}-\not{x_1})(\not{y}-\not{z})(\not{z}-\not{x}_2)s_2\\
\end{aligned}\end{equation}

Note that these in fact show that if we want to contract in the field at $y$ (implicitly contracting the spin structures) the two structures $\<\bar{S}_1 S_y\>\cdot \<\bar{S}_y S_2\>$, we can simply make the replacement $\ket{S_y}\bra{\bar{S}_y} \to \not{P}_y$.

Contracting a pair of structures in embedding space is the same as doing a spin sum between them; this is again the same as replacing $\sum_S \ket{S_3}\bra{S_3} \to \not{P_3}$.


\section{Shadows}

Let us define in general dimension our conventions.

Fermions: $\psi \chi = \psi^\alpha \chi_\alpha = - \chi_\alpha \psi^\alpha = - t \chi^\alpha \psi_\alpha = - t \chi \psi$, for some $t=\pm 1$. See Freedman's supergravity; $t$ depends on the signature and the dimension.

We can sum up an operator by saying it transforms in the representation $V_{\Delta,\rho}$. It only has a non-zero two-point function with operators living in $V_{\Delta,\rho^\dagger}$, with $\rho^\dagger = (\rho^R)^*$, the dual of $\rho^R$. In Lorentzian signature, $\rho^\dagger$ is the conjugate of $\rho$.

Let us say that the shadow transform is defined by applying $\expval{[V_{\tilde\Delta, \rho^R}][V_{\tilde\Delta, \rho^*}]}$ (which is non-zero, since $((\rho^R)^R)^* = \rho^*$) to $[V_{\Delta,\rho}]$ from the left. Thus:
\begin{equation}\begin{aligned}
S[\cO](x) = \int_y \expval{\tilde\cO(x) \tilde\cO^\dagger(y)} \cO(y) \sim V_{\tilde\Delta,\rho^R} \times (\underbrace{V_{\tilde\Delta, \rho^*} \leftrightarrow V_{\Delta, \rho}}_{=\mathrm{id}}) \sim V_{\tilde\Delta, \rho^R}\\
S[\tilde\cO](x) = \int_y \expval{\cO(x) \cO^\dagger(y)} \tilde\cO(y) \sim V_{\Delta,\rho} \times (\underbrace{V_{\Delta, \rho^\dagger} \leftrightarrow V_{\tilde\Delta, \rho^R}}_{=\mathrm{id}}) \sim V_{\Delta, \rho}
\end{aligned}\end{equation}
since $(\rho^R)^* = \rho^\dagger$.
\begin{equation}\begin{aligned} %
S[\cO^\dagger](x) = \int_y \expval{\tilde\cO^\dagger(x) \tilde\cO(y)} \cO^\dagger(y) \sim V_{\tilde\Delta,\rho^*} \times (\underbrace{V_{\tilde\Delta, \rho^R} \leftrightarrow V_{\Delta, \rho^\dagger}}_{=\mathrm{id}}) \sim V_{\tilde\Delta, \rho^*}\\
S[\tilde\cO^\dagger](x) = \int_y \expval{\cO^\dagger(x) \cO(y)} \tilde\cO^\dagger(y) \sim V_{\Delta,\rho^\dagger} \times (\underbrace{V_{\Delta, \rho} \leftrightarrow V_{\tilde\Delta, \rho^*}}_{=\mathrm{id}}) \sim V_{\Delta, \rho^\dagger}
\end{aligned}\end{equation}
Now, we take as convention opposite to \cite{Albayrak:2020rxh} that the shadow contraction acts \cancel{from the left} as follows: \LFT{This may be unwise.}
\begin{equation}\begin{aligned}
S[\cO]_\alpha &= \int \expval{\tilde\cO_\alpha (\tilde{O}^\dagger)^\beta} \expval{\cdots \cO_\beta \cdots},& \quad
S[\tilde\cO]_\alpha &= \int \expval{\tilde\cO_\alpha (\cO^\dagger)^\beta} \expval{\cdots \tilde\cO_\beta \cdots}\\
S[\cO^\dagger]^\alpha &= \int \expval{(\tilde\cO^\dagger)^\alpha (\tilde{O})_\beta} \expval{\cdots (\cO^\dagger)^\beta \cdots}, &\quad
S[\tilde\cO^\dagger]^\alpha &= \int \expval{(\cO^\dagger)^\alpha \cO_\beta} \expval{\cdots (\tilde\cO^\dagger)^\beta \cdots}
\end{aligned}\end{equation}
Note that this is opposite to the real fermions of \cite{Albayrak:2020rxh} (2.5) $S[\cO](x) = \int_y \cO(y) \expval{\tilde\cO(x) \tilde\cO(y)}$, but is the same as the (suppressed indices) \cite{Karateev:2018oml} $S[\cO](x) = \int_y\expval{\tilde\cO(x) \tilde\cO(y)} \cO(y) $.

\section{Calculating shadow coefficients}

We take as conventions, first that the shadow transform always acts by multiplying the two-point function from the left. %
With the convention that the two-point function has coefficient 1, we have the following:
(note that we ignore the linearly dependent $f^{(2)}_{\half\half l}$, as mentioned above):

We know the form of the three point function of two spin zero operators $\phi_{1}$ and $\phi_{2}$ with dimensions $\Delta_1$ and $\Delta_2$ and a spin $J$ operator $O_{\Delta,J}$ is: 
 \begin{equation}\label{eq:threedirect}
 \begin{split}
    \Braket{\phi_1(x_1) \phi_2(x_2) O_{\Delta,J;\bar \mu}(x_3) }
  & = C^{\Delta_1,\Delta_2}_{\Delta,J} \; 
   \frac{  Z_{\mu_1} \dots Z_{\mu_J}  - {\rm traces} }{|x_{12}|^{\Delta_1 + \Delta_2 - \Delta + J}
     |x_{13}|^{\Delta + \Delta_1 -\Delta_2 - J } 
     |x_{23}|^{\Delta + \Delta_2 - \Delta_1 - J} 
   } \;,
   \crcr
   Z_{\mu} &=   \left( \frac{ (x_{13})_{\mu}}{ |x_{13}|^2} 
     - \frac{(x_{23})_{\mu}}{|x_{23}|^2} \right)   \; ,
 \end{split}
 \end{equation}
where $C^{\Delta_1,\Delta_2}_{\Delta,J}$ are pure numbers. Recall that we define $CS$ to be the conformal structure with the OPE coefficients set to one. The shadow coefficient is simply
\begin{equation}\label{eq:Sdef}
\begin{split}
&  \int d^dy \; 
\Braket{ \tilde O_{\tilde \Delta,J;\bar \nu}(x_1) 
\tilde O_{\tilde \Delta,J}^{\bar \mu}(y)    }^{\rm cs}  
 \Braket{ O_{\Delta,J;\bar \mu} (y)   O_2(x_2) O_3 (x_3) }^{\rm cs}  =\crcr
 & \qquad \qquad = 
S^{O_2O_3}_{O} \Braket{ \tilde O_{\tilde \Delta,J;\bar \nu}(x_1) O_2(x_2) O_3(x_3) }^{\rm cs} 
\; ,
\end{split}
\end{equation}
where from now on we assume we deal with real fields (otherwise the spin representation should be conjugated).  We have for instance \cite{Liu:2018jhs}:


==> 99-9-2PI.tex <==
\section{2PI action hunt}
We can write down the Lagrangian of this large-$N$ theory, in the melonic limit, which resembles the SYK model\footnote{We use $\int_{\mathbb{R}^N} d^Nx\text{e}^{-\frac{1}{2}x^TAx+J^Tx}=\frac{\left(2\pi\right)^{N/2}e^{\frac{1}{2}J^2}}{\sqrt{\det A}}$ for $N\times N$ symmetric invertible real matrices $A$, which we generalise to the Euclidean $\int\mathcal{D}\varphi\text{e}^{\int\left(-\frac{1}{2} \varphi A\varphi+J\varphi\right)d^Dx}=\text{e}^{\frac{1}{2}J^2}\sqrt{\det D}$ with $D:=A^{-1}$ for an invertible operator $A$. We also use $\int D\bar{\psi}D\psi e^{-\iint d^4x' d^4x \bar{\psi}(x')B(x',x)\psi(x)} = \det B$; note the minus signs here. Note also that we have used a real $\varphi$ but a complex fermion.}.

\textbf{Conventions being used are commented out here}

Let us begin with an SYK-like model of a $q$-index scalar field in Euclidean space, $\phi_{a_1 a_2 \ldots a_q} = a_q$, transforming in the global $\mathrm{O}(N)^q$:
\begin{equation}
    \int d^dx \half \partial_\mu\phi_A(x) \partial_\mu\phi_A(x) - \frac{\lambda}{S} O_T \phi_A \phi_B \phi_C \phi_D
\end{equation}
We then introduce symmetric bilocal fields $B(x,y)$ and $\Sigma(x,y)$, with $\Sigma$ a Lagrange multiplier field enforcing $B(x,y) =\frac{1}{N^q} \sum_A \phi_A(x) \phi_A(y)$.

\textit{The precise steps between here are not worked out yet. It may involve the 2PI formalism \url{https://arxiv.org/pdf/1808.00612.pdf}, or perhaps the replica trick. However, we know that what we have written below does give the correct SDEs as EL equations.}
We obtain:
\begin{align}
    S_E &= \int d^dx \half \phi_A(x) \left(-\partial^2_{x} \right)\phi_A(x) + \half \int d^D x d^D y \left( \phi_A(x)\Sigma(x,y)\phi_A(y) - N^q B(x,y)\Sigma(x,y) + \frac{\lambda^2 N^{2q}}{S^2} B(x,y)^q\right) (signs)
\end{align}
Integrating out the $N^q$ fields $\phi_A$, which appears only quadratically, we obtain:
\begin{align}
    \frac{S_{eff}}{N^q} &= \half \log\det\left(-\partial^2_{x}\delta(x-y)+ \Sigma(x,y) \right) + \half\int d^D x d^D y \left(- B(x,y)\Sigma(x,y) + \frac{\lambda^2 N^{q}}{S^2} B(x,y)^q\right).
\end{align}
We know that $[\log \det X)]' =(X^{-1})^T$ for $X$ with positive determinant. Thus, if we neglect $\partial_x^2$ (i.e. taking the IR limit), and take the semiclassical saddle point in the $N\to\infty$ limit (assuming $\lambda^2 N^q = \lambda_t^2$ is constant), we obtain as E-L equations the following:
\begin{align}
    0&=\pdv{N^q S_{\text{eff}}}{B(x,y)} = -\Sigma(x,y) + \frac{q \lambda^2}{ S^2} B(x,y)^{q-1} =0\\
    0&=\pdv{N^q S_{\text{eff}}}{\Sigma(x,y)} = (\Sigma(x,y)^{-1})^T - B(x,y) =0\\
   (A^T)^{-1} = (A^{-1})^T \implies& B(x,y)(\Sigma(x,y))^T =1 (????)
\end{align}
This is then apparently equal to \LFT{(show this- likely involves a Fourier transform)}
\begin{align}
    \Sigma(x,y) = \frac{q\lambda^2}{S^2} B(x,y)^{q-1}, &\quad   \int d^d z B(x,z) G(z,y) = \delta(x-y) 
    \end{align}
These are invariant under the following reparametrisations, for $\Delta=1/q$ and $\mathbf{J}_f(z) = \abs{\det(\pdv{z'}{z})}$ the Jacobian determinant for the coordinate change $z'=f(z)$:
\begin{align}
    B(x,y) \to (\mathbf{J}_f(x) \mathbf{J}_f(y))^\Delta B(f(x), f(y)),\quad \Sigma(x,y) \to (\mathbf{J}_f(x) \mathbf{J}_f(y))^{\Delta(q-1)} \Sigma(f(x), f(y))
\end{align}
The invariance of the first is trivial; the invariance of the second relies on the change-of-basis $\int d^d z \mathbf{J}_f(z) = \int d^d z'$ as well as the formula for the Dirac delta function $\delta(z) = \frac{\delta(z')}{\mathbf{J}_f(z)}$ for $z' =f(z)$.

Now, let us perform a linearised reparametrisation, $f(x) = x + \epsilon(x) + O(\epsilon^2)$
Under this transformation, we have:
\begin{align}
J_f(x)  & = \det(\frac{\delta(x + \epsilon(x))}{\delta x}) = 1 + \tr(\frac{\delta \epsilon(x)}{\delta x}) + O(\epsilon^2) = 1+\partial_\mu \epsilon^\mu (x) + O(\epsilon^2)\\
B(x,y) &\to B(x,y) + \Delta B(x,y) (\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))  + (\epsilon^\mu(x) \partial^x_\mu + \epsilon^\mu(y) \partial^y_\mu)B(x,y) + O(\epsilon^2)
\end{align}
Now we substitute $B(x,y)=\int d^d a d^d b \delta(x-a)\delta(x-b) B(a,b)$, in order to be able to perform the functional derivative, and also integrate the second term by parts, neglecting the boundary terms:
\begin{align*}
B'(x,y)&=\int d^d a d^d b \, B(a,b) \delta(x-a)\delta(y-b) \left(1+\Delta(\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))\right)\\
&+ \int d^d a d^d b\, B(a,b)(\delta(y-b)\epsilon^\mu(x) \partial^x_\mu\delta(x-a) + \delta(x-a)\epsilon^\mu(y) \partial^y_\mu \delta(y-b)) + O(\epsilon^2)\\
B'(x,y)&=\int d^d a d^d b \, B(a,b) \delta(x-a)\delta(y-b) \left(1+(\Delta-1)(\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))\right)\\
\frac{\delta B'(x,y)}{\delta B(a,b)} &=\delta(x-a)\delta(y-b) \left(1+(\Delta-1)(\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))\right) + O(\epsilon^2)\\
&\det_{a,b,x,y}(\delta(x-a) \delta(y-b)) = 1, \quad \det_{a,b}(f(x,y))= f(x,y)\\
\implies \det_{a,b,x,y}\left(\frac{\delta B'(x,y)}{\delta B(a,b)}\right) &=\det_{x,y}\left(1+(\Delta-1)(\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))+O(\epsilon^2)\right)\\
\implies \det_{a,b,x,y}\left(\frac{\delta \Sigma'(x,y)}{\delta \Sigma(a,b)}\right) &= \text{"", with } \Delta \to \Delta(q-1)\\
\implies \det_{a,b,x,y}&\left(\frac{\delta B'(x,y)}{\delta B(a,b)} \frac{\delta \Sigma'(x,y)}{\delta \Sigma(a,b)}\right) = \det_{x,y}\left(1+(\Delta q -2)(\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))+O(\epsilon^2)\right)\\
\end{align*}
Let us now identify the change in the action  $S_{eff}$ due to this variation. It is easy to see the change in the non-determinant part is
\begin{align*}
\frac{\delta S_{\text{no }\det}}{N^q} &= \half \int d^D x \int d^D y \left(- B(x,y)\Sigma(x,y) + \frac{\lambda^2 N^{2q}}{S^2} B(x,y)^q\right) \Delta q (\partial^x_\mu \epsilon^\mu(x) +\partial^y_\mu \epsilon^\mu(y))\\
&+ \half \int d^D x \int d^D y \left((\epsilon^\mu(x) \partial^x_\mu + \epsilon^\mu(y) \partial^y_\mu)(- B(x,y)\Sigma(x,y) + \frac{\lambda^2 N^{2q}}{S^2} B(x,y)^{q})\right)\\
&= \half(1-\Delta q) \int d^D x \int d^D y \left((\epsilon^\mu(x) \partial^x_\mu + \epsilon^\mu(y) \partial^y_\mu)(- B(x,y)\Sigma(x,y) + \frac{\lambda^2 N^{2q}}{S^2} B(x,y)^{q})\right)
\end{align*}
The change in the determinant part (neglecting the derivative) is precisely
\begin{align}
    \log\det(\Sigma')-\log\det(\Sigma) = ...
\end{align}
Thus, the partition function:
\begin{align}
    Z[J_B, J_\Sigma] &= \int D B' D\Sigma' \exp\left[ -S(B', \Sigma') + \int_{x,y} J_B(x,y) B'(x,y) + J_\Sigma(x,y) \Sigma'(x,y)\right]\\
\end{align}
From \url{https://arxiv.org/pdf/1604.07818.pdf}, recall:
\begin{quote}
Thus we can view reparametrization invariance as an emergent symmetry of the infrared theory which is spontaneously broken by the conformal solution $G_c$. The zero modes in the action can be viewed as Nambu-Goldstone modes for the spontaneous breaking of the full conformal symmetry down to SL(2, R). Note that we could consider an alternative model which does not have a reparametrization invariance, then we do not get any enhanced contribution in the IR, see appendix (H).
\end{quote}

